Automatic Synthesis of Light Processing Functions for Programmable Photonics: Theory and Realization

Linear light processing functions (e.g., routing, splitting, filtering) are key functions requiring configuration to implement on a programmable photonic integrated circuit (PPIC). In recirculating waveguide meshes (which include loop-backs), this is usually done manually. Some previous results describe explorations to perform this task automatically, but their efficiency or applicability is still limited. In this paper, we propose an efficient method that can automatically realize configurations for many light processing functions on a square-mesh PPIC. At its heart is an automatic differentiation subroutine built upon analytical expressions of scattering matrices, that enables gradient descent optimization for functional circuit synthesis. Similar to the state-of-the-art synthesis techniques, our method can realize configurations for a wide range of light processing functions, and multiple functions on the same PPIC simultaneously. However, we do not need to separate the functions spatially into different subdomains of the mesh, and the resulting optimum can have multiple functions using the same part of the mesh. Furthermore, compared to non-gradient or numerical differentiation based methods, our proposed approach achieves 3x time reduction in computational cost.

==> Automatic Programmable Photonics - Photonics Research 2022 (For Submission) (6)/response.tex <==
\onecolumn

\centerline{\Large{\textbf{Reply to Reviewer's Comments}}}
\vspace{6pt}

We thank all reviewers for their thorough review of the paper and the constructive remarks. Based on the comments from all reviewers, we have carefully revised the paper with the following major changes.

\begin{itemize}
    \item We add more explanations on how to deal with non-idealities (e.g., thermal cross-talk, process variation, dispersion, or beamsplitter error). For instance, we show how to adapt our method when thermal cross-talk is considered, and how to refine the proposed compact model when process variation is present.
    \item We add further numerical results. First, we compare the run-time of our method with non-gradient and numerical differentiation methods, demonstrating the superiority of our approach. Second, we include several different synthesized results under random initialization to show the robustness of our method.
    \item We revise a number of claims made in the original submission, and include several missing references.
\end{itemize}

All modifications in the revised paper are marked in {\color{red}{RED}} color. In what follows, we list detailed responses to all questions posed by the reviewers.

 
\vspace{6pt}
\noindent\textbf{\large Reviewer~\#1}
\vspace{6pt}

\textbf{Q0.} The authors show an effective and efficient method to implement arbitrary configurations on a general purpose programmable photonic integrated circuit. Starting from the theoretical inference of the scattering matrices, a cost function (i.e., error between the actual transfer function of the circuit and the desired one) is defined. Global minimum is found by analytically computing its gradient.  
The concept is interesting, the paper is well written, and the mathematical treatment is very accurate, however the reviewer thinks that there are some aspects that must be thoroughly addressed, before further consideration. 

\vspace{4pt}
% I think the issue is not gradient descent, it's that we don't know the convexity of the loss function. If it's convex, then gradient descent would be able to find the global optimum (to whatever desired residual).
\ans{Thanks for the nice overall summary of our paper and the encouraging words. Before replying to the raised concerns, we want to clarify that gradient descent optimization with non-convex cost functions (and hence our proposed method, where the loss is not necessarily convex) is known to be able to only find local optima. For our applications, however, we typically do not need a global optimum: a local optimal configuration is sufficient. This is also pointed out by Reviewer~\#2. Please refer to our response to his/her Q1 for more details. Below we respond to each raised concern.}
\vspace{4pt}

\textbf{Q1.} The concept related to analytical gradient is of high impact and it is the key message of the paper. Nevertheless, the reviewer cannot find any comparison between the proposed approach and the state-of-the-art methods (mostly based on numerical differentiation). Moreover, in table 1 “run time” column is reported. There are no sufficient details to correctly evaluate this figure of merit (e.g., which kind of system performed the computation? Is 110 minutes acceptable? How far is this number from the performance of state-of-the-art algorithms executed by the same machine?).

\vspace{4pt}
\ans{Thanks for the constructive remark. We agree with the reviewer that a numerical comparison with the state-of-the-art methods (i.e., non-gradient and numerical differentiation based approaches) is needed to support our main contribution. For this goal, we implemented two baseline methods: (i) differential evolution, a population-based gradient-free global optimization approach, and (ii) gradient descent optimization with numerical differentiation. For fairness of comparison, all numerical experiments are performed on the same RedHat Linux server with 16 Intel Xeon E7-4850 CPUs working at 2.1GHz. We add Table~\ref{tab:runtime_comparison} listing the run-time of our method and the baseline methods. It demonstrates that our method achieves more than \improve x time cost reduction compared to the baseline methods. We add this to the discussion in the Numerical Results section.}
\vspace{4pt}

\textbf{Q2.} The last sentence of the abstract is “… (ii) our method is suited to a wide range of light processing functions and can synthesize multiple functions on the same PPIC simultaneously”. The reviewer believes that, as written, it seems to be a novelty claim from the authors’ side. Obviously, the concept of PPICs realizing many different functions has been already demonstrated, for example in refs. [22] and [23] (main text), correctly cited.

\vspace{4pt}
\ans{Thanks for pointing out the concern with this wording and claim. We replace the original last sentence in the abstract with three sentences. The first and the second sentences state that similar to the state-of-the-art synthesis techniques, our method can realize configurations for a wide range of light processing functions and multiple functions on the same PPIC simultaneously. However, we don't need to separate the functions spatially into different subdomains of the mesh, and the resulting optimum can even have multiple functions using the same part of the mesh. The last sentence describes our advantage: a \improve x run-time cost reduction, compared to non-gradient or numerical differentiation based methods.}
\vspace{4pt}

\textbf{Q3.} This work is all about theoretical simulations. The reviewer wonders how the treatment changes if in presence of real actuators (e.g., heaters) with their own non-ideal behaviour (thermal cross-talk). Single derivative dCost/d$\phi$ (and/or dCost/d$\theta$ ) becomes dependent to other phases variations and for sure the complexity of the technique rises. Is it still convenient with respect to conventional numerical methods?

\vspace{4pt}
\ans{Thanks for the thoughtful comment. Our method is still applicable with minor modifications when non-idealities of actuators are taken into account, when those non-idealities can be modeled as differentiable functions. In our paper, we take phase shifts as the design variables, which is a simplification of the real-world scenario, where phase shifts are typically controlled by electrical or thermal actuation. In the case of thermally controlled phased shifters, the delivered power becomes the independent design variable at the lowest level. Without considering the non-idealities of the actuators (e.g., thermal cross-talk of heaters), taking phase shifts or the delivered power as the design variable works equally well in our approach, because no correlation is introduced when mapping from the delivered power to phase shifts or vice versa.}

\ans{However, if thermal cross-talk is considered, we can take the delivered power as the optimized variable, and our method extends naturally to account for thermal cross-talk. Specifically, the original optimization problem shown in Eq.~(\ref{eq:cost}) should now be performed with respect to the delivered power as shown in Eq.~(\ref{eq:cost_thermal})-(\ref{eq:cost_thermal2}) in the added Appendix~\ref{sec:appendixd}. A similar treatment can be adopted for other actuator non-idealities.}

\ans{To better address the concern, we add Appendix~\ref{sec:appendixd} explaining how to apply our method with thermal cross-talk as an example. We also add a paragraph in the 'Dealing with non-ideality' subsection of the Conclusion section, further emphasizing it.}
\vspace{4pt}

\textbf{Q4.} The reviewer agrees with the authors about the statement in line 405, i.e. “Real waveguides do have dispersion, but this does not affect the method, as long as the dispersion of neff can be described by an analytically derivable function”. However, considering neff=ng is too coarse approximation (at least for a paper of this tenure) that hides one the most detrimental drawbacks of PPICs, the narrow FSR.  neff=ng does not hold for high refractive index contrast platforms, which can only be exploited to implement this kind of photonic circuits, in a reasonable footprint. Introduction of neff vs lambda dependence in the theoretical derivation (perhaps in the appendix?) may be helpful for interested readers and could definitely complete the dissertation (supporting also what is written in section 6, paragraph “Dealing with non-ideality”).

\vspace{4pt}
\ans{Thanks for the thoughtful feedback. We would like to address the concern from the following three aspects. First, we respectfully point out that we have treated $n_{\text{eff}}$ as a function of $\omega$ in derivation (e.g., Eq.~(\ref{eq:our_compact_S}) and the first line under it), and only set it to a constant $n_{\text{eff}}=2.35$ in numerical experiments. In other words, dispersion effect has already been considered throughout our derivation. In fact, whether $n_{\text{eff}}$ is frequency dependent or independent only makes a difference when running the circuit simulation: using $n_{\text{eff}}(\omega_k)$ or a constant $n_{\text{eff}}$ at a frequency point $\omega_k$. But it doesn't change the form of any equations ahead of the Numerical Results section.}

\ans{Second, as pointed out by the reviewer, setting $n_{\text{eff}}$ to a constant (i.e., without considering dispersion effect) is not realistic for high refractive contrast platforms and hides the drawback of PPIC --- the narrow FSR. We rephrase the reviewer's comments and add them at the beginning of the Numerical Results section, alerting the readers.}

\ans{Third, we include an example of using our proposed method when dispersion effect is considered here to better address the reviewer's concern. Specifically, we consider synthesizing responses akin to a ring resonator on a three-by-two square mesh under the conditions $n_{\text{eff}}=2.35$ and $n_g=4.0$ at 1550 nm. The desired magnitude and phase responses are shown in (a) and (c) below, and the synthesized responses are correspondingly shown in (b) and (d). They show good agreement, justifying the validity of our proposed method when the dispersion effect is considered. More importantly, the free spectral range (FSR) in this synthesized result is about $0.04 \text{Thz}=40 \text{Ghz}$. Comparing it to the FSRs shown in Table.~\ref{table:details_experiments}, we note that it coincides with the reviewer's comment that FSR is usually narrow when dispersion effect is considered. We are working on a follow-up extension to our method suitable to arbitrary TBU connections and various non-idealities (e.g., thermal cross-talk, dispersion effect). We will include this example and more in our future follow-up paper.}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/revision_extra_res.jpg}
    \caption*{\ans{Fig. An example of using our proposed method when dispersion effect is considered.}}
    \label{fig:my_label}
\end{figure}

\vspace{4pt}


\newpage
\vspace{6pt}
\noindent\textbf{\large Reviewer~\#2}
\vspace{6pt}

\textbf{Q0.} The authors seek to use automatic differentiation to perform various functionalities on recirculating mesh structures. This is an interesting direction and deserves publication because this has previously only been proposed for feedforward structures. The authors do a very thorough job of defining compact models and discussing how to calculate gradients (although, autograd systems do not necessarily require explicit evaluation of these terms). Finally, they evaluate on a square mesh topology and discuss how specific implementations can be optimized on the device. However, there are some major issues that I believe need to be addressed relating to optimization, practicality for experiment and context:

\vspace{4pt}
\ans{Thanks for the nice overall summary of our paper and the encouraging words. Below we respond to each raised concern. }
\vspace{4pt}

\textbf{Q1.} Getting stuck in local optima? How can we be guaranteed that the result of the optimization is not stuck in a local optimum? I think it would make sense to show multiple initial conditions reaching the same final result to confirm that the optimum is indeed ideal. How would this scale for larger circuits?

\vspace{4pt}
% \ans{Thanks for the constructive comment. Gradient descent optimization is known to be only able to find local minimum. When the cost function is convex, every local minimum becomes a global minimum. However, we speculate that it is unlikely the cost function is convex in our case. Thus, as suggested by the reviewers, verifying that the synthesizes results are robust to random phase initialization is important.}

\ans{Thanks for the constructive comment. Gradient descent optimization with non-convex cost functions is known to be only able to find local optima, and thus the specific configuration coming out of the optimization algorithm will depend strongly on the initial condition. To justify the practical utility of the proposed method, we also need to show that even with different initializations, the optimization routine can always yield a good result. We take Case 1 and 5 as examples, run our method with different initializations, and plot the results in Fig.~\ref{fig:case1_random} and Fig.~\ref{fig:case5_random}, respectively. They demonstrate the robustness of our method to random initialization. Note that for our applications, we don't necessarily need a global optimum, while a local optimal configuration is sufficient. When the circuit size scales up, we would expect the optimization result to be more strongly impacted by the initialization, because more local optima might exist for a higher dimensional optimization problem. These discussions are also added in the Numerical Results section.}

% \ans{To address the reviewer's concern, we show the synthesized results for test case 1, 5 and 6 under different random phase initialization in Fig. xx, xx, and xx.}

\vspace{4pt}

\textbf{Q2.} If there are errors in the various components of a real device used to program these terms, there can be some issues with the optimization. I would like the authors to implement or at least comment on the effects of loss and TBU beamsplitter errors in the compact model. Given the fact that this is a recirculating model, how accurate can we expect this approach to be in the presence of nonidealities, which ultimately is a practical consideration we need to make? The authors do have an explanation on “Deal[ing] with non-ideality” however I think a bit more (work or explanation) is needed here to really demonstrate the practicality of this protocol, especially when dealing with recirculating light during tuning of these devices. In addition to dispersion, process variation (loss variation and beamsplitter error variation (systematic vs random)) should be considered by modifying the TBU compact model to incorporate them and rerunning the optimizations in these circumstances. 

I would like the authors to comment if this approach can actually be used to EXTRACT nonidealities from a recirculating circuit given experimental data? If so, that would make this method even more powerful.

\vspace{4pt}
\ans{Thanks for the constructive remark. We first want to respectfully point out that the loss in the TBU (regardless of the loss source) is collectively considered in our parameter $\alpha$. Regarding the beamsplitting error, we have not considered them in our paper: namely, we assume the beamsplitter achieves perfect 50\%:50\% splitting. However, we can borrow Eqs. (1)-(2) from Ref. [9] to take the non-ideality of the beamsplitter into consideration. Note that this won't change any mathematical derivation, but it does change numerical results. The reviewer might be also interested in a similar question asked by Reviewer \#1. In his/her Q4, we comment on the effect of another non-ideality, dispersion, and implement a numerical experiment to verify the validity of our approach. Second, as also posed by Reviewer \#1, we now add explanations on how to adjust our method when thermal cross-talk, another kind of major non-ideality, is considered. Please refer to our response to his/her Q3 for more details. Third, we agree with the reviewer that the compact model needs to be refined when non-ideality is considered. We add Appendix E illustrating how to adapt our compact model for non-ideality (especially considering process variation).}


\ans{Regarding the last question about extraction, we do have an approach to inversely extract the model parameter $\alpha$, though it doesn't use our proposed method. We briefly illustrate the idea here. We set all tunable basic units (TBUs) to cross state. Then the magnitude transmission from an input to an output equals $\alpha^{n}$, where $n$ represents the number of TBUs on this optical path and $\alpha$ represents the TBU loss. Thus, if we can measure the magnitude transmission, we can inversely calculate $\alpha$. In reality, extra careful considerations need to be taken for this extraction method to work. We thank the reviewer for bringing up this question, and we will investigate along this line in our future work.}

\ans{To address the reviewer's concern, we add Appendix D and E, and more explanations in the 'Dealing with non-ideality' subsection. We hope to submit a follow-up paper adapting the proposed method to arbitrary TBU connections and incorporating various non-idealities (such as dispersion and thermal cross-talk).}

% Assume we are dealing with a $N$-by-$M$ square mesh (so there are $(4N+4M)$ outer nodes and $(2N+2M)$ optical paths). First, set all tunable basic units (TBUs) to cross state. Then measure the magnitude transmission of the $(2N+2M)$ optical signals in dB unit and calculate their summation, denoted as $s$. Then our model parameter $\alpha=\exp(\frac{s}{2N+2M+4NM})$

\vspace{4pt}

\textbf{Q3.} It needs better context with recent developments in the literature. Missing references: (i) On tuning recirculating meshes via self-configuration: Multipurpose self-configuration of programmable photonic circuits. Nat Commun 11, 6359 (2020). https://doi.org/10.1038/s41467-020-19608-w; (ii) On optimization theory in feedforward systems: Matrix optimization on universal unitary photonic devices, Physical review applied 11 (6), 064044.

Finally, I would also like the authors to comment on two recent optimization *implementations* implemented in the experimental domain, explained in the following two arxiv articles: (i) https://arxiv.org/abs/2205.08501, (ii) https://arxiv.org/abs/2208.01623. Can this technique be expected to leverage either of these optimization techniques or both in the experimental domain? I am particularly interested in if 2208.01623 applies because it is model free and evidently a bit easier to implement on a single optical layer.

\vspace{4pt}
\ans{Thanks for bringing these two related papers to our attention. They are added in the revised manuscript. Regarding the two arXiv papers, they are very interesting. We would like to first clarify two things and then answer the reviewer's question in the end.}

\ans{\textbf{Structure and application difference}: Note that their programmable photonic circuit structures are both feed-forward, while ours is recirculating. Several particular feed-forward structures (e.g., Reck's and Clement's) are proven to be able to realize any unitary matrix, so a feed-forward programmable photonic circuit is usually exploited to implement Optical Neural Networks (ONNs) for AI computing. Alternatively, a recirculating programmable photonic circuit can realize a ring resonator due to its loop-back connection, and thus, is usually used for optical applications (e.g., fast prototyping photonic integrated circuit).}

\ans{\textbf{Gradient calculation difference}: Training an ONN is done by first defining a cost function and then optimizing it by gradient descent optimization, where gradients are analytically calculated via back propagation. In the mentioned two arXiv papers, they aim to do in-situ ONN training and each propose a way to implement back-propagation in the optical context. 2208.01623 uses a stochastic error-descent approach (see its Fig.4 (b) and Appendix~V). 2205.08501 uses the adjoint method (see its Section~D). Similar to these two works, we have a cost function and gradient descent optimization is used as well. But we differ from them in how to calculate gradients. Specifically, we express the tunable basic unit (TBU) as an analytical model, so that gradients can be directly calculated. }

\ans{\textbf{Our answer}: With the above clarified, we now answer the reviewer's questions. In our understanding, we could use the optical back propagation proposed in these two arXiv papers in the experimental domain for our case, because we believe that adopting their methods from a feed-forward structure to our recirculating structure doesn't affect their applicability. Furthermore, we agree with the reviewer that 2208.06123 is easier to implement on real hardware than our method.}

\ans{However, we want to explain our motivation from the following aspects. First, we use the analytical model of a tunable basic unit (TBU) because we want to get mathematical intuition about the form of transfer functions, as depicted in Section 3 of the main text. Second, when a programmable photonic chip is fabricated, we could do device-level characterization precisely measuring the values of all parameters in the model, so that our synthesis method, which is built upon this model, could be carried out accurately. This is a common procedure known as inverse measurement or characterization, frequently used in literature and also discussed in the previous question Q2. Third, we understand the reviewer's concern about the implementation difficulty of our approach. Recently, we have a follow-up thought which could further simplify our approach and make it suitable to arbitrary TBU connections. Roughly, we believe one could formulate the simulation of a programmable photonic circuit as solving a matrix equation $\mathbf{Ax}=\mathbf{b}$, where $\mathbf{x}$ represents the complex magnitudes at all nodes in the concerned circuit required to solve, and $\mathbf{A}$ and $\mathbf{b}$ could be built following certain principles. Then the gradient of $\mathbf{x}$ with respect to an arbitrary parameter $q\in\{\theta,\phi\}$ is given by: $\frac{d\mathbf{x}}{d q} = -\mathbf{A}^{-1}\frac{d\mathbf{A}}{d q}\mathbf{x}$. With this one-line formula (whose complexity is comparable to 2208.06123's), we could easily obtain all gradients. We are working on this alternative approach and hope to submit a follow-up paper.}

\ans{To address the reviewer's concern, we add the two mentioned arXiv papers into our paper and include a short discussion in the Introduction section.}

\vspace{4pt}

\vspace{6pt}
\noindent\textbf{\large Pre-Production Review}
\vspace{6pt}

\textbf{Q1.} Authors are now required to include a Data Availability Statement in their manuscript file. Details on the new policy can be found at https://opg.optica.org/submit/review....

\vspace{4pt}
\ans{We have added the Data Availability statement in the revised manuscript.}
\vspace{4pt}

\textbf{Q2.} Footnotes (notes at the bottom of text pages) are not used in our journals. Footnotes should be incorporated into the text or set at the back with references as an endnote. Please see the style guide at https://opg.optica.org/submit/style...

\vspace{4pt}
\ans{We have moved footnotes into the main text.}
\vspace{4pt}

\textbf{Q3.} For free color figures online-only please submit electronic art files following instructions given at the journal website: https://opg.optica.org/submit/style...

\vspace{4pt}
\ans{We have corrected the format of our electronic figures.}
\vspace{4pt}

\textbf{Q4.} Please confirm that all of your funding sources have been added into your Prism submission in the Fees and Funding step. If your manuscript is accepted for publication, the Funding listing in your published paper will be pulled from this section.

\vspace{4pt}
\ans{We confirm all funding sources are clearly stated.}
\vspace{4pt}

\textbf{Q5.} Please ensure that all references, figures and tables are called out in the text. Please also check the ordering of your reference, figure and table call outs. If they are out of order it could cause delays with publishing your article.

\vspace{4pt}
\ans{We confirm all reference, figures, and tables are called out correctly.}
\vspace{4pt}

\textbf{Q6.} Please replace et al with all authors in your reference list. In references with 20 or more authors, the author list should be truncated after the first three names and followed by et al.

\textbf{Q7.} After revision, please make sure that the references are cited in numerical order; renumber references if necessary. Please remove any duplicate references and renumber accordingly.

\vspace{4pt}
\ans{We double-check the reference list, ensuring its numbering and format are correct.}
\vspace{4pt}

\clearpage
\twocolumn

==> Automatic Programmable Photonics - Photonics Research 2022 (For Submission) (6)/response2.tex <==
\onecolumn

\centerline{\Large{\textbf{Reply to Reviewer's Comments}}}
\vspace{6pt}

We thank all reviewers for their thorough review of the paper and the constructive remarks. We are encouraged that the questions posted by Reviewer~\#1 and the format issues raised by pre-production review were successfully addressed by our revision. In response to the additional questions raised by Reviewer~\#2, we have made the following major changes:

\begin{itemize}
    \item (For Q1) We added the reference mentioned by the reviewer and discussed it in the paper.
    \item (For Q2, Q3, Q4) We have re-plotted all figures according to the reviewer's suggestions.
\end{itemize}

Below we respond in detail to the remaining questions posed by Reviewer~\#2.

\vspace{6pt}
\noindent\textbf{\large Reviewer~\#2}
\vspace{6pt}

\textbf{Q0. I think the reviewers have answered most of my core concerns, nice work. I do have some minor comments that should be addressed prior to publication...} 

\vspace{4pt}
\ans{Thanks for the encouraging words. Below we respond to the remaining questions.}
\vspace{4pt}

\textbf{Q1. Another reference: would like a brief comment on this paper "Scalable analysis for arbitrary photonic integrated waveguide meshes," (Perez, Capmany Optica, 2019) as it may be related to discussion in the section on "Other PPIC connection topologies."} 

\vspace{4pt}
\ans{Thanks for bringing this paper to our attention. It is highly relevant to our work and has been incorporated as reference [26] in our revised paper. Although reference [26] and our work share some similarities, such as the use of analytical model-based techniques and mathematical induction to derive a system-level transfer function, there are also some differences. For example, they use the analytical result assisted by Monte Carlo to do error calculation or error calibration by utilizing unused parts, with no mentioning or use of analytical gradients. On the other hand, we calculate and utilize analytical gradients for automatic functional synthesis, which is untouched and mentioned as a future topic in reference [26] (as evidenced by its saying `A final interesting application of the method to be explored is synthesis algorithms' in its Section 4). Additionally, their example is a hexagonal mesh, whereas ours is a square mesh. To better address the reviewer's concern, we have added the above discussion in both the introduction section and the 'Other PPIC connection topologies' subsection at the end of our paper.}

\vspace{4pt}

\textbf{Q2. On Fig 13: it probably makes sense to focus on the configurations (the left column seems redundant or can be overlay in a single plot or with reference to fig 6). } 

\vspace{4pt}
\ans{Thanks for the constructive remark. We have re-plotted the left column of Fig. 13. Specifically, we replaced the magnitude response figures with the configuration figures. Although it is not asked, we have re-plotted the right column of Fig. 14 in the same spirit.}
\vspace{4pt}


\textbf{Q3. On phase shift heatmaps: please clarify the phase shifter heatmaps (what they are referring to based on location in circuit). using the twilight cyclic heatmap instead of rainbow might make it clearer whether there is an interesting pattern in the phase shifter heatmap. } 

\vspace{4pt}
\ans{Thank you for the valuable feedback. In response to the first suggestion, we have added clarifications regarding the plotting of the heatmap using the location of phase shifters in a newly added Appendix section C. As for the second suggestion, we would like to respectfully acknowledge that our original heatmaps were already utilizing a cyclic color bar, specifically a HSV cyclic color bar. However, to comply with the reviewer's recommendation, we have now switched to using a twilight cyclic heatmap.}
\vspace{4pt}


\textbf{Q4.General comment: the figure axes / titles could be made larger (roughly the size of the caption text). some of the numbers in the figures have poor contrast and are hard to see (esp the power coupling ratio labels on many figures). } 

\vspace{4pt}
\ans{Thank you for the constructive feedback. In response, we have increased the font size of the text in the axes, titles, and annotations in our figures. Regarding the power coupling ratio, we have not only enlarged the font size, but also increased the transparency of the gray background color to improve contrast between the black annotations and the gray bounding boxes.}

% Zhengqi: not sure if we should finish with a sentence like: Please note that we have taken into consideration the limitations of font size as increasing it further may result in overlapping numbers, as demonstrated in Figure 12 (d), for example.

\vspace{4pt}


\clearpage
\twocolumn

==> response.tex <==
\onecolumn

\centerline{\Large{\textbf{Reply to Reviewer's Comments}}}
\vspace{6pt}

We thank all reviewers for their thorough review of the paper and the constructive remarks. Based on the comments from all reviewers, we have carefully revised the paper with the following major changes.

\begin{itemize}
    \item We add more explanations on how to deal with non-idealities (e.g., thermal cross-talk, process variation, dispersion, or beamsplitter error). For instance, we show how to adapt our method when thermal cross-talk is considered, and how to refine the proposed compact model when process variation is present.
    \item We add further numerical results. First, we compare the run-time of our method with non-gradient and numerical differentiation methods, demonstrating the superiority of our approach. Second, we include several different synthesized results under random initialization to show the robustness of our method.
    \item We revise a number of claims made in the original submission, and include several missing references.
\end{itemize}

All modifications in the revised paper are marked in {\color{red}{RED}} color. In what follows, we list detailed responses to all questions posed by the reviewers.

 
\vspace{6pt}
\noindent\textbf{\large Reviewer~\#1}
\vspace{6pt}

\textbf{Q0.} The authors show an effective and efficient method to implement arbitrary configurations on a general purpose programmable photonic integrated circuit. Starting from the theoretical inference of the scattering matrices, a cost function (i.e., error between the actual transfer function of the circuit and the desired one) is defined. Global minimum is found by analytically computing its gradient.  
The concept is interesting, the paper is well written, and the mathematical treatment is very accurate, however the reviewer thinks that there are some aspects that must be thoroughly addressed, before further consideration. 

\vspace{4pt}
% I think the issue is not gradient descent, it's that we don't know the convexity of the loss function. If it's convex, then gradient descent would be able to find the global optimum (to whatever desired residual).
\ans{Thanks for the nice overall summary of our paper and the encouraging words. Before replying to the raised concerns, we want to clarify that gradient descent optimization with non-convex cost functions (and hence our proposed method, where the loss is not necessarily convex) is known to be able to only find local optima. For our applications, however, we typically do not need a global optimum: a local optimal configuration is sufficient. This is also pointed out by Reviewer~\#2. Please refer to our response to his/her Q1 for more details. Below we respond to each raised concern.}
\vspace{4pt}

\textbf{Q1.} The concept related to analytical gradient is of high impact and it is the key message of the paper. Nevertheless, the reviewer cannot find any comparison between the proposed approach and the state-of-the-art methods (mostly based on numerical differentiation). Moreover, in table 1 “run time” column is reported. There are no sufficient details to correctly evaluate this figure of merit (e.g., which kind of system performed the computation? Is 110 minutes acceptable? How far is this number from the performance of state-of-the-art algorithms executed by the same machine?).

\vspace{4pt}
\ans{Thanks for the constructive remark. We agree with the reviewer that a numerical comparison with the state-of-the-art methods (i.e., non-gradient and numerical differentiation based approaches) is needed to support our main contribution. For this goal, we implemented two baseline methods: (i) differential evolution, a population-based gradient-free global optimization approach, and (ii) gradient descent optimization with numerical differentiation. For fairness of comparison, all numerical experiments are performed on the same RedHat Linux server with 16 Intel Xeon E7-4850 CPUs working at 2.1GHz. We add Table~\ref{tab:runtime_comparison} listing the run-time of our method and the baseline methods. It demonstrates that our method achieves more than \improve x time cost reduction compared to the baseline methods. We add this to the discussion in the Numerical Results section.}
\vspace{4pt}

\textbf{Q2.} The last sentence of the abstract is “… (ii) our method is suited to a wide range of light processing functions and can synthesize multiple functions on the same PPIC simultaneously”. The reviewer believes that, as written, it seems to be a novelty claim from the authors’ side. Obviously, the concept of PPICs realizing many different functions has been already demonstrated, for example in refs. [22] and [23] (main text), correctly cited.

\vspace{4pt}
\ans{Thanks for pointing out the concern with this wording and claim. We replace the original last sentence in the abstract with three sentences. The first and the second sentences state that similar to the state-of-the-art synthesis techniques, our method can realize configurations for a wide range of light processing functions and multiple functions on the same PPIC simultaneously. However, we don't need to separate the functions spatially into different subdomains of the mesh, and the resulting optimum can even have multiple functions using the same part of the mesh. The last sentence describes our advantage: a \improve x run-time cost reduction, compared to non-gradient or numerical differentiation based methods.}
\vspace{4pt}

\textbf{Q3.} This work is all about theoretical simulations. The reviewer wonders how the treatment changes if in presence of real actuators (e.g., heaters) with their own non-ideal behaviour (thermal cross-talk). Single derivative dCost/d$\phi$ (and/or dCost/d$\theta$ ) becomes dependent to other phases variations and for sure the complexity of the technique rises. Is it still convenient with respect to conventional numerical methods?

\vspace{4pt}
\ans{Thanks for the thoughtful comment. Our method is still applicable with minor modifications when non-idealities of actuators are taken into account, when those non-idealities can be modeled as differentiable functions. In our paper, we take phase shifts as the design variables, which is a simplification of the real-world scenario, where phase shifts are typically controlled by electrical or thermal actuation. In the case of thermally controlled phased shifters, the delivered power becomes the independent design variable at the lowest level. Without considering the non-idealities of the actuators (e.g., thermal cross-talk of heaters), taking phase shifts or the delivered power as the design variable works equally well in our approach, because no correlation is introduced when mapping from the delivered power to phase shifts or vice versa.}

\ans{However, if thermal cross-talk is considered, we can take the delivered power as the optimized variable, and our method extends naturally to account for thermal cross-talk. Specifically, the original optimization problem shown in Eq.~(\ref{eq:cost}) should now be performed with respect to the delivered power as shown in Eq.~(\ref{eq:cost_thermal})-(\ref{eq:cost_thermal2}) in the added Appendix~\ref{sec:appendixd}. A similar treatment can be adopted for other actuator non-idealities.}

\ans{To better address the concern, we add Appendix~\ref{sec:appendixd} explaining how to apply our method with thermal cross-talk as an example. We also add a paragraph in the 'Dealing with non-ideality' subsection of the Conclusion section, further emphasizing it.}
\vspace{4pt}

\textbf{Q4.} The reviewer agrees with the authors about the statement in line 405, i.e. “Real waveguides do have dispersion, but this does not affect the method, as long as the dispersion of neff can be described by an analytically derivable function”. However, considering neff=ng is too coarse approximation (at least for a paper of this tenure) that hides one the most detrimental drawbacks of PPICs, the narrow FSR.  neff=ng does not hold for high refractive index contrast platforms, which can only be exploited to implement this kind of photonic circuits, in a reasonable footprint. Introduction of neff vs lambda dependence in the theoretical derivation (perhaps in the appendix?) may be helpful for interested readers and could definitely complete the dissertation (supporting also what is written in section 6, paragraph “Dealing with non-ideality”).

\vspace{4pt}
\ans{Thanks for the thoughtful feedback. We would like to address the concern from the following three aspects. First, we respectfully point out that we have treated $n_{\text{eff}}$ as a function of $\omega$ in derivation (e.g., Eq.~(\ref{eq:our_compact_S}) and the first line under it), and only set it to a constant $n_{\text{eff}}=2.35$ in numerical experiments. In other words, dispersion effect has already been considered throughout our derivation. In fact, whether $n_{\text{eff}}$ is frequency dependent or independent only makes a difference when running the circuit simulation: using $n_{\text{eff}}(\omega_k)$ or a constant $n_{\text{eff}}$ at a frequency point $\omega_k$. But it doesn't change the form of any equations ahead of the Numerical Results section.}

\ans{Second, as pointed out by the reviewer, setting $n_{\text{eff}}$ to a constant (i.e., without considering dispersion effect) is not realistic for high refractive contrast platforms and hides the drawback of PPIC --- the narrow FSR. We rephrase the reviewer's comments and add them at the beginning of the Numerical Results section, alerting the readers.}

\ans{Third, we include an example of using our proposed method when dispersion effect is considered here to better address the reviewer's concern. Specifically, we consider synthesizing responses akin to a ring resonator on a three-by-two square mesh under the conditions $n_{\text{eff}}=2.35$ and $n_g=4.0$ at 1550 nm. The desired magnitude and phase responses are shown in (a) and (c) below, and the synthesized responses are correspondingly shown in (b) and (d). They show good agreement, justifying the validity of our proposed method when the dispersion effect is considered. More importantly, the free spectral range (FSR) in this synthesized result is about $0.04 \text{Thz}=40 \text{Ghz}$. Comparing it to the FSRs shown in Table.~\ref{table:details_experiments}, we note that it coincides with the reviewer's comment that FSR is usually narrow when dispersion effect is considered. We are working on a follow-up extension to our method suitable to arbitrary TBU connections and various non-idealities (e.g., thermal cross-talk, dispersion effect). We will include this example and more in our future follow-up paper.}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/revision_extra_res.jpg}
    \caption*{\ans{Fig. An example of using our proposed method when dispersion effect is considered.}}
    \label{fig:my_label}
\end{figure}

\vspace{4pt}


\newpage
\vspace{6pt}
\noindent\textbf{\large Reviewer~\#2}
\vspace{6pt}

\textbf{Q0.} The authors seek to use automatic differentiation to perform various functionalities on recirculating mesh structures. This is an interesting direction and deserves publication because this has previously only been proposed for feedforward structures. The authors do a very thorough job of defining compact models and discussing how to calculate gradients (although, autograd systems do not necessarily require explicit evaluation of these terms). Finally, they evaluate on a square mesh topology and discuss how specific implementations can be optimized on the device. However, there are some major issues that I believe need to be addressed relating to optimization, practicality for experiment and context:

\vspace{4pt}
\ans{Thanks for the nice overall summary of our paper and the encouraging words. Below we respond to each raised concern. }
\vspace{4pt}

\textbf{Q1.} Getting stuck in local optima? How can we be guaranteed that the result of the optimization is not stuck in a local optimum? I think it would make sense to show multiple initial conditions reaching the same final result to confirm that the optimum is indeed ideal. How would this scale for larger circuits?

\vspace{4pt}
% \ans{Thanks for the constructive comment. Gradient descent optimization is known to be only able to find local minimum. When the cost function is convex, every local minimum becomes a global minimum. However, we speculate that it is unlikely the cost function is convex in our case. Thus, as suggested by the reviewers, verifying that the synthesizes results are robust to random phase initialization is important.}

\ans{Thanks for the constructive comment. Gradient descent optimization with non-convex cost functions is known to be only able to find local optima, and thus the specific configuration coming out of the optimization algorithm will depend strongly on the initial condition. To justify the practical utility of the proposed method, we also need to show that even with different initializations, the optimization routine can always yield a good result. We take Case 1 and 5 as examples, run our method with different initializations, and plot the results in Fig.~\ref{fig:case1_random} and Fig.~\ref{fig:case5_random}, respectively. They demonstrate the robustness of our method to random initialization. Note that for our applications, we don't necessarily need a global optimum, while a local optimal configuration is sufficient. When the circuit size scales up, we would expect the optimization result to be more strongly impacted by the initialization, because more local optima might exist for a higher dimensional optimization problem. These discussions are also added in the Numerical Results section.}

% \ans{To address the reviewer's concern, we show the synthesized results for test case 1, 5 and 6 under different random phase initialization in Fig. xx, xx, and xx.}

\vspace{4pt}

\textbf{Q2.} If there are errors in the various components of a real device used to program these terms, there can be some issues with the optimization. I would like the authors to implement or at least comment on the effects of loss and TBU beamsplitter errors in the compact model. Given the fact that this is a recirculating model, how accurate can we expect this approach to be in the presence of nonidealities, which ultimately is a practical consideration we need to make? The authors do have an explanation on “Deal[ing] with non-ideality” however I think a bit more (work or explanation) is needed here to really demonstrate the practicality of this protocol, especially when dealing with recirculating light during tuning of these devices. In addition to dispersion, process variation (loss variation and beamsplitter error variation (systematic vs random)) should be considered by modifying the TBU compact model to incorporate them and rerunning the optimizations in these circumstances. 

I would like the authors to comment if this approach can actually be used to EXTRACT nonidealities from a recirculating circuit given experimental data? If so, that would make this method even more powerful.

\vspace{4pt}
\ans{Thanks for the constructive remark. We first want to respectfully point out that the loss in the TBU (regardless of the loss source) is collectively considered in our parameter $\alpha$. Regarding the beamsplitting error, we have not considered them in our paper: namely, we assume the beamsplitter achieves perfect 50\%:50\% splitting. However, we can borrow Eqs. (1)-(2) from Ref. [9] to take the non-ideality of the beamsplitter into consideration. Note that this won't change any mathematical derivation, but it does change numerical results. The reviewer might be also interested in a similar question asked by Reviewer \#1. In his/her Q4, we comment on the effect of another non-ideality, dispersion, and implement a numerical experiment to verify the validity of our approach. Second, as also posed by Reviewer \#1, we now add explanations on how to adjust our method when thermal cross-talk, another kind of major non-ideality, is considered. Please refer to our response to his/her Q3 for more details. Third, we agree with the reviewer that the compact model needs to be refined when non-ideality is considered. We add Appendix E illustrating how to adapt our compact model for non-ideality (especially considering process variation).}


\ans{Regarding the last question about extraction, we do have an approach to inversely extract the model parameter $\alpha$, though it doesn't use our proposed method. We briefly illustrate the idea here. We set all tunable basic units (TBUs) to cross state. Then the magnitude transmission from an input to an output equals $\alpha^{n}$, where $n$ represents the number of TBUs on this optical path and $\alpha$ represents the TBU loss. Thus, if we can measure the magnitude transmission, we can inversely calculate $\alpha$. In reality, extra careful considerations need to be taken for this extraction method to work. We thank the reviewer for bringing up this question, and we will investigate along this line in our future work.}

\ans{To address the reviewer's concern, we add Appendix D and E, and more explanations in the 'Dealing with non-ideality' subsection. We hope to submit a follow-up paper adapting the proposed method to arbitrary TBU connections and incorporating various non-idealities (such as dispersion and thermal cross-talk).}

% Assume we are dealing with a $N$-by-$M$ square mesh (so there are $(4N+4M)$ outer nodes and $(2N+2M)$ optical paths). First, set all tunable basic units (TBUs) to cross state. Then measure the magnitude transmission of the $(2N+2M)$ optical signals in dB unit and calculate their summation, denoted as $s$. Then our model parameter $\alpha=\exp(\frac{s}{2N+2M+4NM})$

\vspace{4pt}

\textbf{Q3.} It needs better context with recent developments in the literature. Missing references: (i) On tuning recirculating meshes via self-configuration: Multipurpose self-configuration of programmable photonic circuits. Nat Commun 11, 6359 (2020). https://doi.org/10.1038/s41467-020-19608-w; (ii) On optimization theory in feedforward systems: Matrix optimization on universal unitary photonic devices, Physical review applied 11 (6), 064044.

Finally, I would also like the authors to comment on two recent optimization *implementations* implemented in the experimental domain, explained in the following two arxiv articles: (i) https://arxiv.org/abs/2205.08501, (ii) https://arxiv.org/abs/2208.01623. Can this technique be expected to leverage either of these optimization techniques or both in the experimental domain? I am particularly interested in if 2208.01623 applies because it is model free and evidently a bit easier to implement on a single optical layer.

\vspace{4pt}
\ans{Thanks for bringing these two related papers to our attention. They are added in the revised manuscript. Regarding the two arXiv papers, they are very interesting. We would like to first clarify two things and then answer the reviewer's question in the end.}

\ans{\textbf{Structure and application difference}: Note that their programmable photonic circuit structures are both feed-forward, while ours is recirculating. Several particular feed-forward structures (e.g., Reck's and Clement's) are proven to be able to realize any unitary matrix, so a feed-forward programmable photonic circuit is usually exploited to implement Optical Neural Networks (ONNs) for AI computing. Alternatively, a recirculating programmable photonic circuit can realize a ring resonator due to its loop-back connection, and thus, is usually used for optical applications (e.g., fast prototyping photonic integrated circuit).}

\ans{\textbf{Gradient calculation difference}: Training an ONN is done by first defining a cost function and then optimizing it by gradient descent optimization, where gradients are analytically calculated via back propagation. In the mentioned two arXiv papers, they aim to do in-situ ONN training and each propose a way to implement back-propagation in the optical context. 2208.01623 uses a stochastic error-descent approach (see its Fig.4 (b) and Appendix~V). 2205.08501 uses the adjoint method (see its Section~D). Similar to these two works, we have a cost function and gradient descent optimization is used as well. But we differ from them in how to calculate gradients. Specifically, we express the tunable basic unit (TBU) as an analytical model, so that gradients can be directly calculated. }

\ans{\textbf{Our answer}: With the above clarified, we now answer the reviewer's questions. In our understanding, we could use the optical back propagation proposed in these two arXiv papers in the experimental domain for our case, because we believe that adopting their methods from a feed-forward structure to our recirculating structure doesn't affect their applicability. Furthermore, we agree with the reviewer that 2208.06123 is easier to implement on real hardware than our method.}

\ans{However, we want to explain our motivation from the following aspects. First, we use the analytical model of a tunable basic unit (TBU) because we want to get mathematical intuition about the form of transfer functions, as depicted in Section 3 of the main text. Second, when a programmable photonic chip is fabricated, we could do device-level characterization precisely measuring the values of all parameters in the model, so that our synthesis method, which is built upon this model, could be carried out accurately. This is a common procedure known as inverse measurement or characterization, frequently used in literature and also discussed in the previous question Q2. Third, we understand the reviewer's concern about the implementation difficulty of our approach. Recently, we have a follow-up thought which could further simplify our approach and make it suitable to arbitrary TBU connections. Roughly, we believe one could formulate the simulation of a programmable photonic circuit as solving a matrix equation $\mathbf{Ax}=\mathbf{b}$, where $\mathbf{x}$ represents the complex magnitudes at all nodes in the concerned circuit required to solve, and $\mathbf{A}$ and $\mathbf{b}$ could be built following certain principles. Then the gradient of $\mathbf{x}$ with respect to an arbitrary parameter $q\in\{\theta,\phi\}$ is given by: $\frac{d\mathbf{x}}{d q} = -\mathbf{A}^{-1}\frac{d\mathbf{A}}{d q}\mathbf{x}$. With this one-line formula (whose complexity is comparable to 2208.06123's), we could easily obtain all gradients. We are working on this alternative approach and hope to submit a follow-up paper.}

\ans{To address the reviewer's concern, we add the two mentioned arXiv papers into our paper and include a short discussion in the Introduction section.}

\vspace{4pt}

\vspace{6pt}
\noindent\textbf{\large Pre-Production Review}
\vspace{6pt}

\textbf{Q1.} Authors are now required to include a Data Availability Statement in their manuscript file. Details on the new policy can be found at https://opg.optica.org/submit/review....

\vspace{4pt}
\ans{We have added the Data Availability statement in the revised manuscript.}
\vspace{4pt}

\textbf{Q2.} Footnotes (notes at the bottom of text pages) are not used in our journals. Footnotes should be incorporated into the text or set at the back with references as an endnote. Please see the style guide at https://opg.optica.org/submit/style...

\vspace{4pt}
\ans{We have moved footnotes into the main text.}
\vspace{4pt}

\textbf{Q3.} For free color figures online-only please submit electronic art files following instructions given at the journal website: https://opg.optica.org/submit/style...

\vspace{4pt}
\ans{We have corrected the format of our electronic figures.}
\vspace{4pt}

\textbf{Q4.} Please confirm that all of your funding sources have been added into your Prism submission in the Fees and Funding step. If your manuscript is accepted for publication, the Funding listing in your published paper will be pulled from this section.

\vspace{4pt}
\ans{We confirm all funding sources are clearly stated.}
\vspace{4pt}

\textbf{Q5.} Please ensure that all references, figures and tables are called out in the text. Please also check the ordering of your reference, figure and table call outs. If they are out of order it could cause delays with publishing your article.

\vspace{4pt}
\ans{We confirm all reference, figures, and tables are called out correctly.}
\vspace{4pt}

\textbf{Q6.} Please replace et al with all authors in your reference list. In references with 20 or more authors, the author list should be truncated after the first three names and followed by et al.

\textbf{Q7.} After revision, please make sure that the references are cited in numerical order; renumber references if necessary. Please remove any duplicate references and renumber accordingly.

\vspace{4pt}
\ans{We double-check the reference list, ensuring its numbering and format are correct.}
\vspace{4pt}

\clearpage
\twocolumn

==> response2.tex <==
\onecolumn

\centerline{\Large{\textbf{Reply to Reviewer's Comments}}}
\vspace{6pt}

We thank all reviewers for their thorough review of the paper and the constructive remarks. We are encouraged that the questions posted by Reviewer~\#1 and the format issues raised by pre-production review were successfully addressed by our revision. In response to the additional questions raised by Reviewer~\#2, we have made the following major changes:

\begin{itemize}
    \item (For Q1) We added the reference mentioned by the reviewer and discussed it in the paper.
    \item (For Q2, Q3, Q4) We have re-plotted all figures according to the reviewer's suggestions.
\end{itemize}

Below we respond in detail to the remaining questions posed by Reviewer~\#2.

\vspace{6pt}
\noindent\textbf{\large Reviewer~\#2}
\vspace{6pt}

\textbf{Q0. I think the reviewers have answered most of my core concerns, nice work. I do have some minor comments that should be addressed prior to publication...} 

\vspace{4pt}
\ans{Thanks for the encouraging words. Below we respond to the remaining questions.}
\vspace{4pt}

\textbf{Q1. Another reference: would like a brief comment on this paper "Scalable analysis for arbitrary photonic integrated waveguide meshes," (Perez, Capmany Optica, 2019) as it may be related to discussion in the section on "Other PPIC connection topologies."} 

\vspace{4pt}
\ans{Thanks for bringing this paper to our attention. It is highly relevant to our work and has been incorporated as reference [26] in our revised paper. Although reference [26] and our work share some similarities, such as the use of analytical model-based techniques and mathematical induction to derive a system-level transfer function, there are also some differences. For example, they use the analytical result assisted by Monte Carlo to do error calculation or error calibration by utilizing unused parts, with no mentioning or use of analytical gradients. On the other hand, we calculate and utilize analytical gradients for automatic functional synthesis, which is untouched and mentioned as a future topic in reference [26] (as evidenced by its saying `A final interesting application of the method to be explored is synthesis algorithms' in its Section 4). Additionally, their example is a hexagonal mesh, whereas ours is a square mesh. To better address the reviewer's concern, we have added the above discussion in both the introduction section and the 'Other PPIC connection topologies' subsection at the end of our paper.}

\vspace{4pt}

\textbf{Q2. On Fig 13: it probably makes sense to focus on the configurations (the left column seems redundant or can be overlay in a single plot or with reference to fig 6). } 

\vspace{4pt}
\ans{Thanks for the constructive remark. We have re-plotted the left column of Fig. 13. Specifically, we replaced the magnitude response figures with the configuration figures. Although it is not asked, we have re-plotted the right column of Fig. 14 in the same spirit.}
\vspace{4pt}


\textbf{Q3. On phase shift heatmaps: please clarify the phase shifter heatmaps (what they are referring to based on location in circuit). using the twilight cyclic heatmap instead of rainbow might make it clearer whether there is an interesting pattern in the phase shifter heatmap. } 

\vspace{4pt}
\ans{Thank you for the valuable feedback. In response to the first suggestion, we have added clarifications regarding the plotting of the heatmap using the location of phase shifters in a newly added Appendix section C. As for the second suggestion, we would like to respectfully acknowledge that our original heatmaps were already utilizing a cyclic color bar, specifically a HSV cyclic color bar. However, to comply with the reviewer's recommendation, we have now switched to using a twilight cyclic heatmap.}
\vspace{4pt}


\textbf{Q4.General comment: the figure axes / titles could be made larger (roughly the size of the caption text). some of the numbers in the figures have poor contrast and are hard to see (esp the power coupling ratio labels on many figures). } 

\vspace{4pt}
\ans{Thank you for the constructive feedback. In response, we have increased the font size of the text in the axes, titles, and annotations in our figures. Regarding the power coupling ratio, we have not only enlarged the font size, but also increased the transparency of the gray background color to improve contrast between the black annotations and the gray bounding boxes.}

% Zhengqi: not sure if we should finish with a sentence like: Please note that we have taken into consideration the limitations of font size as increasing it further may result in overlapping numbers, as demonstrated in Figure 12 (d), for example.

\vspace{4pt}


\clearpage
\twocolumn
